Convex Optimization of Linear Impulsive Rendezvous

This note aims at providing a concise and self-contained document that describes a clear and easy-to-understand method, that could be useful for a reader that is approaching the linear-impulsive rendezvous topic for the first time, but that is also flexible enough to accommodate problem variations, such as additional constraints like bounded-magnitude DV, or direction constraints with minor modifications.

==> Tables/data_atv3.tex <==
\begin{tabular}{c c} 
\hline 
Parameter & Value \\ 
\hline 
$a$ (km) & \num{6763.00} \\ 
$e$ & \num{0.0052} \\ 
$i$ (deg) & \num{52.00} \\ 
$\Omega$ (deg) & \num{0.00} \\ 
$\omega$ (deg) & \num{0.00} \\ 
$\theta_0$ (deg) & \num{0.00} \\ 
$\Delta t$ (s) & \num{55350} \\ 
\hline 
\end{tabular} 


==> Tables/data_prisma.tex <==
\begin{tabular}{c c} 
\hline 
Parameter & Value \\ 
\hline 
$a$ (km) & \num{7011.00} \\ 
$e$ & \num{0.004} \\ 
$i$ (deg) & \num{98.00} \\ 
$\Omega$ (deg) & \num{190.00} \\ 
$\omega$ (deg) & \num{0.00} \\ 
$\theta_0$ (deg) & \num{0.00} \\ 
$\Delta t$ (s) & \num{64620} \\ 
\hline 
\end{tabular} 


==> Tables/results_four_impulse.tex <==
\begin{tabular}{c c c c}
\hline
Parameter & Carter & Convex & Optimal \\ 
\hline
$\theta_1$ & 0 & 0 & 0 \\ 
$\theta_2$ & $\pi / 2 \approx $ 1.5708 & 1.6997 & 1.7077 \\ 
$\theta_3$ & $3 \pi / 2 \approx $ 4.7124 & 4.5835 & 4.5859 \\ 
$\theta_4$ & $2 \pi \approx $ 6.2832 & 6.2832 & 6.2832 \\ 
$\bm{\Delta v}_1$ & $\begin{bmatrix} +0.0273 & -0.0344 \end{bmatrix}$ & $\begin{bmatrix} +0.0263 & -0.0328 \end{bmatrix}$ & $\begin{bmatrix} +0.0266 & -0.0329  \end{bmatrix}$\\ 
$\bm{\Delta v}_2$ & $\begin{bmatrix} -0.0896 & -0.0119 \end{bmatrix}$ & $\begin{bmatrix} -0.0911 & -0.0046 \end{bmatrix}$ & $\begin{bmatrix} -0.0917 & -0.0046  \end{bmatrix}$\\ 
$\bm{\Delta v}_3$ & $\begin{bmatrix} +0.0896 & -0.0119 \end{bmatrix}$ & $\begin{bmatrix} +0.0914 & -0.0045 \end{bmatrix}$ & $\begin{bmatrix} +0.0901 & -0.0043  \end{bmatrix}$\\ 
$\bm{\Delta v}_4$ & $\begin{bmatrix} -0.0273 & -0.0344 \end{bmatrix}$ & $\begin{bmatrix} -0.0263 & -0.0329 \end{bmatrix}$ & $\begin{bmatrix} +0.0259 & -0.0322  \end{bmatrix}$\\ 
Overall $\Delta v$ & 0.2686 & 0.2671 & 0.2667 \\ 
\hline
\end{tabular}


==> Tables/results_prisma.tex <==
\begin{tabular}{c c c c}
\hline
Parameter & Arzelier et al. & Convex & \\ \hline
$\theta_1$ & 0 & 0 \\ 
$\theta_2$ & 3.4071 & 3.39355 \\ 
$\theta_3$ & 69.4999 & 69.4999 \\ 
$\bm{\Delta v}_1 (m/s)$ & $\begin{bmatrix} +0.049110 & -0.001994 \end{bmatrix}$ & $\begin{bmatrix} +0.049113 & -0.002021 \end{bmatrix}$\\ 
$\bm{\Delta v}_2 (m/s)$ & $\begin{bmatrix} +0.002037 & \num{-7e-06} \end{bmatrix}$ & $\begin{bmatrix} +0.002036 & \num{-5.05926e-06} \end{bmatrix}$\\ 
$\bm{\Delta v}_3 (m/s)$ & $\begin{bmatrix} -0.051313 & -0.001466 \end{bmatrix}$ & $\begin{bmatrix} -0.051312 & -0.001498 \end{bmatrix}$\\ 
Overall $\Delta v$ (m/s) & 0.102525 & 0.102525 \\ 
\hline
\end{tabular}


==> Tables/results_three_impulse.tex <==
\begin{tabular}{c c c c}
\hline
Parameter & Carter & Convex & Optimal \\ 
\hline
$\theta_1$ & 0 & 0 & 0 \\ 
$\theta_2$ & $\pi / 2 \approx $ 1.5708 & 2.4053 & 2.4119 \\ 
$\theta_3$ & $2 \pi \approx $ 6.2832 & 6.2832 & 6.2832 \\ 
$\bm{\Delta v}_1$ & $\begin{bmatrix} -1.6294 & +0.6667 \end{bmatrix}$ & $\begin{bmatrix} -1.7767 & +0.3868 \end{bmatrix}$ & $\begin{bmatrix} -1.7776 & +0.3838  \end{bmatrix}$\\ 
$\bm{\Delta v}_2$ & $\begin{bmatrix} -0.3901 & -0.0964 \end{bmatrix}$ & $\begin{bmatrix} -0.2901 & +0.0156 \end{bmatrix}$ & $\begin{bmatrix} -0.2896 & +0.0164  \end{bmatrix}$\\ 
$\bm{\Delta v}_3$ & $\begin{bmatrix} +0.0633 & +0.0259 \end{bmatrix}$ & $\begin{bmatrix} +0.0669 & +0.0146 \end{bmatrix}$ & $\begin{bmatrix} +0.0672 & +0.0145  \end{bmatrix}$\\ 
Overall $\Delta v$ & 2.2308 & 2.1773 & 2.1773 \\ 
\hline
\end{tabular}


==> sez2old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       SEZIONE 2 OLD
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


This note investigates the impulsive time-constrained rendezvous of an active \textit{chaser}  
spacecraft with a passive \textit{target} spacecraft.
We employ the classical Hill-Clohessy-Wiltshire equations for linearized motion
about a circular reference orbit.
Thus, a state transition matrix 
$\Phi(t_k, t_j)$ permits to link any state vector $\bm{x}(t_k)$ with 
one at a later time $\bm{x}(t_j)$ \hl{with/through/according to} 
the following relationship:
\begin{equation}
    \bm{x}(t_j) = \Phi(t_k, t_j) \bm{x}(t_k)
    \label{eq:state_transition_matrix}
\end{equation}

The state of the chaser is fully described by its position $(x, y, z)$ 
and velocity $(v_x, v_y, v_z)$:
\begin{equation*}
    \bm{x} = \begin{bmatrix}
    x & y & z & v_x & v_y & v_z
    \end{bmatrix}
\end{equation*}
The position and velocity of the chaser are 
expressed in a right-handed system centered in the target with the $x$-axis in
the direction of the radius from Earth's center to the target and with the 
$z$-axis in the direction of the angular velocity vector of the target.

The only control on the chaser spacecraft is the thrust.
Since it is modeled as impulsive, instantaneous velocity changes 
are applied to the chaser.
Therefore, the set of control variables is made up by the components of 
the velocity change vector in the aforementioned coordinate system:
\begin{equation}
    \bm{u} = \bm{\Delta v} = \begin{bmatrix}
        \Delta v_x & \Delta v_y & \Delta v_z 
    \end{bmatrix}
\end{equation}
From now on, we will denote with $\Delta v$ the magnitude of the velocity
change vector $\bm{\Delta v}$.

We are interested in the minimum-fuel transfer. 
Hence, we formulate the problem as an optimal control problem
aimed at minimizing the cost function $J$ defined as the overall $\Delta v$:
\begin{equation}
    \min_{\bm{x}, \bm{u}, N, t_j} J = \sum_{j = 1}^{N} \Delta v(t_j)
\end{equation}
where $N$ is the total number of impulses, each one applied at a specific time
$t_j$.
Notice that both the optimal number and time instants of the impulses must be 
determined.

The state variables must satisfy the differential constraints of
Eq.~\eqref{eq:state_transition_matrix}.
Considering the impulsive velocity change, these can be expressed as:
\begin{equation}
    \bm{x}(t_{j + 1}^{-}) = \Phi(t_{j + 1}^{-}, t_{j}^{+}) \bm{x}(t_j^{+}) 
    \qquad \forall j = 1, \dots, N - 1
    \label{eq:differential_con_original}
\end{equation}
where $t_j^{+}$ and $t_j^{-}$ denote respectively the time instant immediately
after and before the application of the impulse $\Delta v(t_j)$.
Thus, \hl{[Questa specificazione si puo togliere se eccessiva.]}
\begin{align}
    x(t_j^+) &= x(t_j^-) \\
    y(t_j^+) &= y(t_j^-) \\
    z(t_j^+) &= z(t_j^-) \\
    v_x(t_j^+) &= v_x(t_j^-) + \Delta v_x(t_j) \\
    v_y(t_j^+) &= v_y(t_j^-) + \Delta v_y(t_j) \\
    v_z(t_j^+) &= v_z(t_j^-) + \Delta v_z(t_j)
\end{align}



